Higher Idempotent Completion for Soergel Bimodules

We present two applications of the concept of higher idempotent completion to higher categories relevant in link homology theory and higher representation theory. We show that singular Soergel bimodules can be recovered from Soergel bimodules through partial 2-categorical idempotent completions. Specializing to type A, we further assemble singular Soergel bimodules into a semistrict monoidal 2-category and identify certain quotients as semistrict monoidal 2-categories of gl_N foams. Our second main result uses 2-categorical idempotent completions to formulate a higher categorical branching rule for such foam theories, which underlie the Lee-Gornik-Rasmussen-Wu deformations of coloured gl_N link homology. In particular, we provide a fully local version of Rose-Wedrich's decomposition theorem on deformed coloured link homology.

==> preamble.tex <==
%auto-ignore
%this ensures the arxiv doesn't try to start TeXing here.
%!TEX root=main.tex
%\input{preferences.tex}

\usepackage{latexsym,exscale,enumerate}
\usepackage{mathtools,mathabx,mathscinet,amsfonts,amssymb,amsthm,bbm,euscript}
%\usepackage{MnSymbol}
\usepackage{amscd, stmaryrd}
\usepackage[normalem]{ulem}
\usepackage[all]{xy}
\SelectTips{cm}{}
\usepackage{graphicx}
\usepackage{wrapfig}
\usepackage{xcolor}
\usepackage{dirtytalk}
\usepackage{bm}
\usepackage{amsmath} % for bigboxtimes
\usepackage{tensor}

%\usepackage{xurl}



%%%%%%%%%%% page formatting %%%%%%%%%%%

\addtolength{\hoffset}{-1.6cm}
\addtolength{\textwidth}{3cm}
\hfuzz=6pc


%%%%%%%%%%% hyperref %%%%%%%%%%%

\RequirePackage{color}
\definecolor{references}{rgb}{.7,.1,.6}

\RequirePackage[pdftex,                                                         
colorlinks = true,                                                              
urlcolor = references, % \href{...}{...} external (URL)                         
citecolor = references, % \cite{...}                                            
linkcolor = references, % \ref{...} and \pageref{...}                           
]
{hyperref}
\usepackage{cleveref}


%%%%%%%%%%% tikz %%%%%%%%%%%


\usepackage{tikz}
\usepackage{tikz-cd}
\usetikzlibrary{math}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{arrows,shapes,positioning}
%%multiple arrow options
\tikzstyle directed=[postaction={decorate,decoration={markings,
    mark=at position #1 with {\arrow{>}}}}]
\tikzstyle rdirected=[postaction={decorate,decoration={markings,
    mark=at position #1 with {\arrow{<}}}}]

\tikzset{anchorbase/.style={baseline={([yshift=-0.5ex]current bounding box.center)}},
    tinynodes/.style={font=\tiny,text height=0.75ex,text depth=0.15ex},
    smallnodes/.style={font=\scriptsize,text height=0.75ex,text depth=0.15ex},
    >={Latex[length=1mm, width=1.5mm]}
  }
  \tikzset{
    partial ellipse/.style args={#1:#2:#3}{
        insert path={+ (#1:#3) arc (#1:#2:#3)}
    }
}
\tikzcdset{arrow style=tikz, diagrams={>=stealth}}

  
\newcommand\mydots{\makebox[1em][c]{$\cdot$\hfil$\cdot$\hfil$\cdot$}}
\newcommand\mysdots{\makebox[.5em][c]{$\cdot$\hfil$\cdot$\hfil$\cdot$}}

\allowdisplaybreaks
\numberwithin{equation}{section}

%%%%%%%%%%% macros %%%%%%%%%%%

%%% color macros %%%

\colorlet{green}{black!30!green}
\newcommand{\BLUE}[1]{\textcolor[rgb]{0.00,0.00,0.80}{#1}}
\newcommand{\GREEN}[1]{\textcolor[rgb]{0.00,0.70,0.00}{#1}}
\newcommand{\RED}[1]{\textcolor[rgb]{0.70,0.00,0.00}{#1}}
\newcommand{\GRAY}[1]{\textcolor[rgb]{0.50,0.50,0.50}{#1}}

%%% bibliography macros %%%
\usepackage[backend=biber,style=alphabetic, doi=false,isbn=false,url=false, maxbibnames=9, maxalphanames=6]{biblatex}
\addbibresource{biblio.bib}
\newcommand{\arxiv}[1]{\href{https://arxiv.org/abs/#1}{\small  arXiv:#1}}
\newcommand{\doi}[1]{\href{https://dx.doi.org/#1}{{\small DOI:#1}}}
\newcommand{\euclid}[1]{\href{https://projecteuclid.org/getRecord?id=#1}{{\small  #1}}}
\newcommand{\mathscinet}[1]{\href{https://www.ams.org/mathscinet-getitem?mr=#1}{\small  #1}}
\newcommand{\googlebooks}[1]{(preview at \href{https://books.google.com/books?id=#1}{google books})}
\newcommand{\notfree}{}
\newcommand{\numdam}[1]{}

\input{sbimtikz.tex}
%%% abbreviations in italics %%%

\def\emph#1{{\sl #1\/}}
\def\ie{{\sl i.e.\;}}
\def\eg{{\sl e.g.\;}}
\def\Eg{{\sl E.g.\/}}
\def\etc{{\sl etc.\/}}
\def\cf{{\sl c.f.\;}}
\def\etal{\sl{et al.\/}}%
\def\vs{\sl{vs.\/}}%


%%% lazyness macros %%%
\def\cal#1{\mathcal{#1}}
\def\mf#1{\mathfrak{#1}}
\def\la{\langle}
\def\ra{\rangle}
\def\lra{{\longrightarrow}}
\let\hat=\widehat
\let\tilde=\widetilde
\newcommand{\ot}{\leftarrow}

\newcommand*{\defeq}{=}
\renewcommand{\to}{\rightarrow}
\newcommand{\To}{\Rightarrow}
\newcommand{\TO}{\Rrightarrow}
\newcommand{\scs}{\scriptsize}

%%% alphabet macros %%%

\def\A{\mathbb{A}}
\def\B{\mathbb{B}}
\def\C{\mathbb{C}}
\def\D{\mathbb{D}}
\def\Eb{\mathbb{E}}
\renewcommand{\L}{\mathbb{L}}
\def\N{\mathbb{N}}
\def\Q{\mathbb{Q}}
\def\R{\mathbb{R}}
\def\T{\mathbb{T}}
\def\U{\mathbb{U}}
\def\V{\mathbb{V}}
\def\W{\mathbb{W}}
\def\X{\mathbb{X}}
\def\Y{\mathbb{Y}}
\def\Z{\mathbb{Z}}

\newcommand{\AS}{\EuScript A}
\newcommand{\BS}{\EuScript B}
%\newcommand{\CS}{\EuScript C}
\newcommand{\CS}{\mathrm{C}}
\newcommand{\Cat}{\mathrm{Cat}}
\newcommand{\CCS}{\mathcal{C}}
\newcommand{\DS}{\EuScript D}
\newcommand{\IS}{\EuScript I}
\newcommand{\JS}{\EuScript J}
\newcommand{\KS}{\EuScript K}
\newcommand{\RS}{\EuScript R}
\newcommand{\TS}{\EuScript T}
\newcommand{\US}{\EuScript U}
\newcommand{\BB}{\mathbf{B}}
\newcommand{\CB}{\mathbf{C}}
\newcommand{\USd}{\dot{\EuScript U}}
\newcommand{\VS}{\EuScript V}
\newcommand{\VSred}{\overline{\EuScript V}}
%\newcommand{\VSred}{\EuScript V'}
% \newcommand{\WS}{\EuScript W}
% \newcommand{\YS}{\EuScript Y}

%%% greek letters %%%

\renewcommand{\a}{\alpha}
\renewcommand{\b}{\beta}
\renewcommand{\d}{\delta}
\newcommand{\e}{\varepsilon}

\newcommand{\thickchi}{\mathcal{X}}
\newcommand{\Chi}{\mathfrak{X}}

%%% algebraic structure macros %%%
\newcommand{\gltwo}{\mf{gl}_2}
\newcommand{\sln}{\mf{sl}_n}
\newcommand{\slN}{\mf{sl}_N}
\newcommand{\slm}{\mf{sl}_m}
\newcommand{\slnn}[1]{\mf{sl}_{#1}}

\newcommand{\gln}{\mf{gl}_N}
\newcommand{\glN}{\mf{gl}_N}
\newcommand{\glm}{\mf{gl}_m}
\newcommand{\glnn}[1]{\mf{gl}_{#1}}
\newcommand{\GLN}{\mathrm{GL}_N}

\newcommand{\Bim}{\mathrm{Bim}}
%\newcommand{\SBim}{\mathrm{SBim}}
\newcommand{\smallsbim}{\mathrm{sBim}}
\newcommand{\sBSbim}{\mathrm{sBSBim}} %bicategory of singular bott-samelsons
\newcommand{\sbsbim}{\mathrm{sBSbim}}
\newcommand{\kkSBim}{\mathrm{Kar}^2 \mathrm{SBim}}
\newcommand{\kksSBim}{\mathrm{Kar}^2\mathrm{sSBim}}
\newcommand{\sbim}{\mathrm{SBim}} %for the bicategory obtained by delooping
\newcommand{\SBim}{\mathrm{Sbim}}  %this is the monoidal 1-category of Soergel bimodules
\newcommand{\BSbim}{\mathrm{BSbim}}
\newcommand{\BSBim}{\mathrm{BSBim}} %delopped Bott Samelsons
\newcommand{\msbim}{\mathbf{SBim}} %monoidal bicat of soergel bimods
\newcommand{\mbsbim}{\mathbf{BSBim}} %monoidal bicat of bott-samelson
\newcommand{\mssbim}{\mathbf{sSBim}} %monoidal bicat of singular soergel bimods
\newcommand{\msbsbim}{\mathbf{sBSBim}} %monoidal bicat of singular BS bimods
\newcommand{\sSbim}{\mathrm{sSBim}} %bicategory of singular soergel bimodules
\newcommand{\SSBim}{\mathrm{SSBim}}
\newcommand{\Hilb}{\mathrm{Hilb}}
\newcommand{\FHilb}{\mathrm{FHilb}}
\newcommand{\symg}{\mathfrak{S}}
\newcommand{\Proj}{\mathrm{Proj}}
\newcommand{\Spec}{\mathrm{Spec}}
\newcommand{\Mod}{\text{-}\mathrm{Mod}}
\newcommand{\Ob}{\mathrm{Ob}}
%\newcommand{\Cat}{\mathbf{Cat}}
\newcommand{\Rep}{\mathbf{Rep}}

%%% elements, objects, morphisms %%%

\newcommand{\coev}{\mathrm{coev}}
\newcommand{\del}{\partial}
\newcommand{\ev}{\mathrm{ev}}
\newcommand{\id}{\mathrm{id}}
\newcommand{\Id}{\mathrm{id}}
\newcommand{\idem}{\mathbbm{1}}
\newcommand{\one}{\mathbbm{1}}
\newcommand{\oone}{\mathbf{1}}
\newcommand{\ooone}{\mathsf{1}}
\newcommand{\tr}{\mathrm{tr}}
\newcommand{\mergemap}{\mathrm{merge_{\mathbf{\underline{n}}}^{\mathbf{\underline{m}}}}}
\newcommand{\splitmap}{\mathrm{split_{\mathbf{\underline{m}}}^{\mathbf{\underline{n}}}}}

%%% operator & functor macros %%%


\newcommand{\ad}{\operatorname{ad}}
\newcommand{\Aut}{\operatorname{Aut}}
\newcommand{\Br}{\operatorname{Br}}
\newcommand{\Ch}{\operatorname{Ch}}
\newcommand{\coker}{{\operatorname{coker}}}
\newcommand{\cone}{\operatorname{cone}}
\newcommand{\convl}{\operatorname{conv}}
\newcommand{\End}{\operatorname{End}}
\newcommand{\END}{\operatorname{END}}
\newcommand{\uEnd}{\underline{\End}}
\newcommand{\Ext}{\operatorname{Ext}}
\newcommand{\twoCat}{\operatorname{2Cat}}

\newcommand{\FT}{\operatorname{FT}}
\newcommand{\HH}{\operatorname{HH}}
\newcommand{\HHH}{\operatorname{HHH}}
\newcommand{\Hom}{\operatorname{Hom}}
\newcommand{\HOM}{\operatorname{HOM}}
\newcommand{\Homcat}{\operatorname{\mathbf{Hom}}}
\newcommand{\Endcat}{\operatorname{\mathbf{End}}}
\newcommand{\uHom}{\underline{\Hom}}
\newcommand{\im}{{\operatorname{im}}}
\newcommand{\Ind}{\operatorname{Ind}}
\newcommand{\Kar}{\operatorname{Kar}}
\newcommand{\Kh}{\operatorname{Kh}}
\newcommand{\CKh}{\operatorname{CKh}}
\newcommand{\KhR}{\operatorname{KhR}}
\newcommand{\largewedge}{\mbox{\Large $\wedge$}}
\newcommand{\Res}{\operatorname{Res}}
\newcommand{\rk}{\operatorname{\rk}}
\newcommand{\spann}{\operatorname{span}}
\newcommand{\Span}{\operatorname{Span}}
\newcommand{\Sym}{\operatorname{Sym}}
\newcommand{\taut}{\operatorname{taut}} 
\newcommand{\Tor}{\operatorname{Tor}}
\newcommand{\Tr}{\operatorname{Tr}}
\newcommand{\vTr}{\operatorname{vTr}}
\newcommand{\hTr}{\operatorname{hTr}}
\newcommand{\tw}{\operatorname{tw}}
\newcommand{\Tw}{\operatorname{Tw}}
\newcommand{\wt}{\operatorname{wt}}
\newcommand{\SB}{\mathrm{SB}}
\newcommand{\kartwobj}[2]{#1[#2]}
\newcommand{\add}[1]{#1^\oplus}


\newcommand{\defFoam}{\Foam_+^{\Sigma}}
\newcommand{\defNFoam}{\NFoam_+^{\Sigma}}
\newcommand{\dotFoam}{\Foam_+^{\bullet}}
\newcommand{\dotNFoam}{\NFoam_+^{\bullet}}
\newcommand{\kdefFoam}{\kar \NFoam_+^{\Sigma}}
\newcommand{\kdefFoaml}{\kar \NFoam_+^{\lambda\in\Sigma}}
\newcommand{\kkdefFoam}{\kkar\kar \NFoam_+^{\Sigma}}


%%% suffix macros %%%

\newcommand{\dmod}{{\mathrm{-mod}}}   %% finitely-generated modules
\newcommand{\dgmod}{-\mathrm{dgmod}}
\newcommand{\fmod}{{\mathrm{-fmod}}}   %% finite-dimensional modules
\renewcommand{\pmod}{{\mathrm{-pmod}}}  %% fin-gen projective modules


%%% sub/superscript macros %%%

\newcommand{\op}{\mathrm{op}}
\newcommand{\co}{\mathrm{co}}
\newcommand{\inv}{^{-1}}
\newcommand{\se}{^{(e)}}
\newcommand{\sh}{^{(h)}}
\newcommand{\dg}{\mathrm{dg}}	
\newcommand{\tot}{\mathrm{tot}}


%%% degree shifts

\newcommand{\adeg}{\mathbf{a}}
\newcommand{\qdeg}{\mathbf{q}}
\newcommand{\tdeg}{\mathbf{t}}


%%% Bar-Natan, TL macros %%%

\newcommand{\kirby}{\omega} % Kirby color, without subscript
\newcommand{\Kirby}{\Omega} % Kirby color, without subscript
\newcommand{\JW}{P} % the Jones-Wenzl, without subscript
\newcommand{\symobj}{\JW} % the symmetric object (in Kar(TL) 
							%or Kar(ABN)), without subscript
\newcommand{\bn}{\mathrm{BN}} % "pre" Bar-Natan category
\newcommand{\BN}{\mathcal{BN}} % Bar-Natan category
\newcommand{\Ann}{\mathcal{A}}
\newcommand{\ABN}{\Ann\BN} % annular Bar-Natan category
\newcommand{\TL}{\mathrm{TL}} % TL category
\newcommand{\dTL}{\mathrm{d}\TL} % dotted TL category
\newcommand{\Pol}{\mathbf{Pol}} % polynomial representation of dotted TL
\newcommand{\KdTL}{\mathrm{Kd}\TL} % Kirbyfied dotted TL category
\newcommand{\Web}{\mathrm{Web}} % Web category
\newcommand{\dWeb}{\mathrm{d}\Web} % dotted Web category
\newcommand{\Sz}{\mathcal{S}_0^N} % skein lasagna module for glN
\newcommand{\Sztwo}{\mathcal{S}_0^2} % skein lasagna module for gl2
\newcommand{\Bproj}{P^{\mathrm{bot}}} %% bottom projectors
\newcommand{\CKproj}{P}	%% Ck projectors
\newcommand{\Comp}{\mathrm{Comp}}	

\newcommand{\addNFoam}{\add{\mathrm{\mathbf{NFoam}}}}

\newcommand{\NFoam}{\mathrm{\mathbf{NFoam}}} %for the non additive version
\newcommand{\Foam}{\mathbf{Foam}} %for the monoidal non additive version

\newcommand{\addFoam}{\add{\mathrm{\mathbf{Foam}}}}

%% some foam macros 

\newcommand{\Nsheet}{\begin{tikzpicture}[anchorbase, line cap = round, scale = 0.5, fill opacity=0.2]
	\path[fill = cl_dark_blue]  (0,0) to (0,2) to (-1.5, 3) to (-1.5, 1) to  (0,0);
	\draw[thick] (0,0) to (0,2) to (-1.5, 3) to (-1.5, 1) to  (0,0);
	\node[black, opacity = 1] at (-0.75, 1.5){\tiny$\bullet^N$};
	\node[black, opacity = 1] at (-1.25, 2.4){\tiny$1$};
\end{tikzpicture}}

\newcommand{\isheet}{\begin{tikzpicture}[anchorbase, line cap = round, scale = 0.5, fill opacity=0.2]
	\path[fill = cl_dark_blue]  (0,0) to (0,2) to (-1.5, 3) to (-1.5, 1) to  (0,0);
	\draw[thick] (0,0) to (0,2) to (-1.5, 3) to (-1.5, 1) to  (0,0);
	\node[black, opacity = 1] at (-0.75, 1.5){\tiny$\bullet^i$};
	\node[black, opacity = 1] at (-1.25, 2.4){\tiny$1$};
\end{tikzpicture}}

%categories 
\newcommand{\Mat}{\mathrm{Mat}} %additive completion
\newcommand{\mat}{\mathrm{Mat}^1}
\newcommand{\mmat}{\mathrm{Mat}^2}
\newcommand{\kar}{\mathrm{Kar}^1}
\newcommand{\kkar}{\mathrm{Kar}^2}

\newcommand{\Set}{\mathrm{Set}} % category of sets
\newcommand{\Vect}{\mathrm{Vect}} % cat. of vector spaces
\newcommand{\fdVect}{\mathrm{fdVect}} % cat. of f.d. vector spaces
\newcommand{\Ai}{A_{\infty}}

\newcommand{\gmod}{\mathrm{-gMod}}
\newcommand{\gbimod}{\mathrm{-gMod-}}


%%%%%%%%%%% Environments %%%%%%%%%%%


\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
\newtheorem{theorem}[thm]{Theorem}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{proposition}[thm]{Proposition}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{corollary}[thm]{Corollary}
%\newtheorem{construction}[thm]{Construction}
\newtheorem{por}[thm]{Porism}
%\newtheorem{principle}[thm]{Principle}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{lemma}[thm]{Lemma}
\newtheorem{goal}[thm]{Goal}
\newtheorem{conj}[thm]{Conjecture}
\newtheorem{hyp}[thm]{Hypothesis}
\theoremstyle{definition}
%\newtheorem{defi}[thm]{Definition}
\newtheorem{definition}[thm]{Definition}
\newtheorem{construction}[thm]{Construction}
%\theoremstyle{remark}
\newtheorem{rem}[thm]{Remark}
\newtheorem{remark}[thm]{Remark}
\newtheorem{obs}[thm]{Observation}
\newtheorem{question}[thm]{Question}
\newtheorem{exas}[thm]{Examples}
\newtheorem{exa}[thm]{Example}
\newtheorem{example}[thm]{Example}
\newtheorem{conv}[thm]{Convention}
\newtheorem*{exa-nono}{Example}
\newtheorem*{theoremA}{Theorem A}
\newtheorem*{theoremB}{Theorem B}
\newtheorem*{theoremC}{Theorem C}
\newtheorem*{theoremD}{Theorem D}

%%%%%%

\newcommand{\Antisym}{\operatorname{Antisym}}
\newcommand{\twoEnd}{\operatorname{2End}}
\newcommand{\powerset}{\cal{P}}


%%%%%%%%%%% Maintenance %%%%%%%%%%%

\newcommand*{\isacomment}{\textcolor{blue}}
\newcommand*{\PW}{\textcolor{green}}

\newcommand{\commented}[1]{}



==> sbimtikz.tex <==
\usepackage{tikz}
\usepackage{tikz-cd}
\usetikzlibrary{math}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{arrows,shapes,positioning, patterns}
\colorlet{green}{black!30!green}


%%color blind adjustments
\definecolor{cl_blue}{HTML}{66CCEE}
\definecolor{cl_red}{HTML}{AA3377}
\definecolor{cl_green}{HTML}{228833}
\definecolor{cl_purple}{HTML}{EE6677}
\definecolor{cl_yellow}{HTML}{FFE200}
\definecolor{cl_dark_blue}{HTML}{0029A9}

%mid arrow command 
\tikzset{
	mid arrow/.style={postaction={decorate,decoration={
				markings,
				mark=at position .5 with {\arrow[#1]{To}}
	}}},
}

\usetikzlibrary{decorations.pathmorphing}

\newcommand\xrsquigarrow[1]{%
\stepcounter{sarrow}%
\begin{tikzpicture}[decoration=snake]
\node (\thesarrow) {\strut\tiny#1};
\draw[->,decorate] (\thesarrow.south west) -- (\thesarrow.south east);
\end{tikzpicture}%
}

%%multiple arrow options
\tikzstyle directed=[postaction={decorate,decoration={markings,
    mark=at position #1 with {\arrow{>}}}}]
\tikzstyle rdirected=[postaction={decorate,decoration={markings,
    mark=at position #1 with {\arrow{<}}}}]

\tikzset{
    anchorbase/.style={baseline={([yshift=-0.5ex]current bounding box.center)}},
    tinynodes/.style={font=\tiny,text height=0.75ex,text depth=0.15ex},
    smallnodes/.style={font=\scriptsize,text height=0.75ex,text depth=0.15ex},
    >={Latex[length=1mm, width=1.5mm]},
    rd/.style={cl_red, line width=.5mm},
    bl/.style={cl_blue, line width=.5mm},
    gr/.style={cl_green, line width=.5mm},
    bla/.style={black, line width=.5mm},
    pu/.style={cl_purple, line width=.5mm},
    gy/.style={gray, line width=.5mm},
    or/.style={orange, line width=.5mm},
    web/.style={very thick},
    dweb/.style={double},
    wh/.style={white,line width=.15cm}
  }
\tikzcdset{arrow style=tikz, diagrams={>=stealth}}
  \newcommand{\ru}{to [out=0,in=270]}
  \newcommand{\rd}{to [out=0,in=90]}
  \newcommand{\ur}{to [out=90,in=180]}
  \newcommand{\uur}{to [out=90,in=225]}
  \newcommand{\uul}{to [out=90,in=315]}
  \newcommand{\ddr}{to [out=270,in=135]}
  \newcommand{\ddl}{to [out=270,in=45]}
  \newcommand{\uru}{to [out=45,in=270]}
  \newcommand{\ulu}{to [out=135,in=270]}
  \newcommand{\ul}{to [out=90,in=0]}
  \newcommand{\lu}{to [out=180,in=270]}
  \newcommand{\ld}{to [out=180,in=90]}
  \newcommand{\dr}{to [out=270,in=180]}
  \newcommand{\dl}{to [out=270,in=0]}
  \newcommand{\pu}{to [out=90,in=270]}
  \newcommand{\pr}{to [out=0,in=180]}
  \newcommand{\pd}{to [out=270,in=90]}
  \newcommand{\pl}{to [out=180,in=0]}



\newcommand{\webA}{

\begin{tikzpicture} [baseline = 1.2cm, line cap = round, scale=.5,fill opacity=0.2]
	\draw[green, very thick, mid arrow] (-3,2.5) to (-4.5,2.5);
	\draw[blue, very thick, mid arrow] (-2,3) to [out=180, in=45] (-3,2.5);
	\draw[blue, very thick, mid arrow] (-4.5,2.5) to [out=135,in=0] (-6,3);
	\draw[red, very thick, mid arrow]  (-1.5,2) to [out=180, in=315] (-3,2.5);
	\draw[red, very thick, mid arrow] (-4.5,2.5) to [out=225,in=0] (-5.5,2);	
\end{tikzpicture}
}

\newcommand{\webB}{
\begin{tikzpicture} [baseline = 1.2cm, line cap = round, scale=.5,fill opacity=0.2]
	\draw[blue, very thick, mid arrow] (-2,3) to (-6,3);
	\draw[red, very thick, mid arrow] (-1.5,2) to  (-5.5,2);	
\end{tikzpicture}
}

\newcommand{\webC}{

\begin{tikzpicture} [baseline = 1.2cm, line cap = round, scale=.5,fill opacity=0.2]
	\draw[green,very thick, mid arrow] (1,2.5) to (-.5,2.5);
	\draw[green, very thick, mid arrow] (-3,2.5) to (-4.5,2.5);
	\draw[red, very thick, mid arrow] (-.5,2.5) to [out=135,in=0] (-2,3) to [out=180, in=45] (-3,2.5);
	\draw[blue, very thick, mid arrow] (-.5,2.5) to [out=225,in=0] (-1.5,2) to [out=180, in=315] (-3,2.5);
\end{tikzpicture}
}


\newcommand{\webD}{
\begin{tikzpicture} [baseline = 1.2cm, line cap = round, scale=.5,fill opacity=0.2]
	\draw[green, very thick, mid arrow] (1,2.5) to (-4.5,2.5);
\end{tikzpicture}
}

\newcommand{\smap}{
	\begin{tikzpicture}[line cap = round, scale=.4]
	\draw [blue, very thick,mid arrow] (2.25,0) to (.75,0);
	\draw [green, very thick,mid arrow] (.75,0) to [out=135,in=0] (-1,.75);
	\draw [red, very thick,mid arrow] (.75,0) to [out=225,in=0] (-4.5,-1.55);
	\draw [orange, very thick,mid arrow] (-1,.75) to [out=135,in=0] (-2.75,1.55);
	\draw [violet, very thick,mid arrow] (-1,.75)to [out=225,in=0] (-4.5,-.25);
	\draw [cyan, very thick,mid arrow] (-2.75,1.55) to [out=135,in=0] (-4.5,2.35);
	\draw [magenta, very thick,mid arrow] (-2.75,1.55)to [out=225,in=0] (-4.5,.55);
\end{tikzpicture}

}


